FlightGoggles: A Modular Framework for Photorealistic Camera, Exteroceptive Sensor, and Dynamics Simulation

FlightGoggles is a photorealistic sensor simulator for perception-driven robotic vehicles. The key contributions of FlightGoggles are twofold. First, FlightGoggles provides photorealistic exteroceptive sensor simulation using graphics assets generated with photogrammetry. Second, it provides the ability to combine (i) synthetic exteroceptive measurements generated in silico in real time and (ii) vehicle dynamics and proprioceptive measurements generated in motio by vehicle(s) in a motion-capture facility. FlightGoggles is capable of simulating a virtual-reality environment around autonomous vehicle(s). While a vehicle is in flight in the FlightGoggles virtual reality environment, exteroceptive sensors are rendered synthetically in real time while all complex extrinsic dynamics are generated organically through the natural interactions of the vehicle. The FlightGoggles framework allows for researchers to accelerate development by circumventing the need to estimate complex and hard-to-model interactions such as aerodynamics, motor mechanics, battery electrochemistry, and behavior of other agents. The ability to perform vehicle-in-the-loop experiments with photorealistic exteroceptive sensor simulation facilitates novel research directions involving, e.g., fast and agile autonomous flight in obstacle-rich environments, safe human interaction, and flexible sensor selection. FlightGoggles has been utilized as the main test for selecting nine teams that will advance in the AlphaPilot autonomous drone racing challenge. We survey approaches and results from the top AlphaPilot teams, which may be of independent interest.

==> cloud_simulation.tex <==
% !TEX root = root.tex

\section{CLOUD SIMULATION}
\label{sec:cloud_simulation}

FlightGoggles can be operated with multiple machines or cloud environments.
In order to obtain photorealistic camera images with high frequency, FlightGoggles often requires high computational resources.
Such computational cost can be achieved by parallel operation of computational resources, e.g. computing machines with multiple GPU or headless servers such as AWS.
The tasks of rendering each camera and updating the vehicles’ dynamics model can be manually assigned to each computational resource.
This parallelization of computation enables FlightGoggles to simulate multiple vehicles with high-resolution camera sensors without significant latency.
The manual to setup cloud simulation environments is included in our confluence page.


\section{PYTHON API}
\label{sec:python_api}
FlightGoggles provides Python API for applications such as deep learning and offline testing and tuning of vision algorithms.
The high-fidelity simulation has been required in the field of machine learning due to the recent success in deep reinforcement learning.
In order to provide convenient integration with existing deep learning framework, e.g. Pytorch or Tensorflow, we implement Python wrappers for all components of FlightGoggles libraries, including the dynamics models and the rendering client.
All scenarios including simulating multiple vehicles or running cloud simulation also can be used with Python API.

Besides utilizing FlightGoggles in machine learning research, we also expect that the Python API can provide a convenient environment for virtual robotics experiments.
The vision algorithms such as visual odometry can be evaluated and tuned on FlightGoggles before operating on the real-world environment.
Moreover, based on FlightGoggles Python API, the online robotics experiments are designed for MIT lecture of autonomous racing cars.


\section{MULTIPLE VEHICLE SIMULATION}
\label{sec:multiple_vehicle_simulation}
FlightGoggles provides a parallel simulation of multiple vehicles. 
Recently, many research has been conducted in the field of swarm navigations which focuses on coordinating multiple vehicles to achieve complicated robotics tasks.
On the other hand, research on non-cooperative motion planning has been conducted which can be applied to racing games.
FlightGoggles is able to operate these experiments online by simulating multiple vehicles with corresponding sensors such as inertial measurement units and cameras.
We provide the dynamics simulation of a dubins car and a multicopter aircraft, and all physical parameters for each vehicle are configurable.

\begin{figure*}
  \centering
  \includegraphics[width=0.96\textwidth]{images/multi_vehicle2.png}
	\label{fig:multi_vehicle}
	\caption{Camera images of multiple vehicles can be parallelly rendered.}
\end{figure*}
